Indirect dark matter searches in the dwarf satellite galaxy Ursa Major II with the MAGIC Telescopes

The dwarf spheroidal galaxy Ursa Major II (UMaII) is believed to be one of the most dark-matter dominated systems among the Milky Way satellites and represents a suitable target for indirect dark matter (DM) searches. The MAGIC telescopes carried out a deep observation campaign on UMaII between 2014 and 2016, collecting almost one hundred hours of good-quality data. This campaign enlarges the pool of DM targets observed at very high energy (E$\gtrsim$50GeV) in search for signatures of dark matter annihilation in the wide mass range between $\sim$100 GeV and $\sim$100 TeV. To this end, the data are analyzed with the full likelihood analysis, a method based on the exploitation of the spectral information of the recorded events for an optimal sensitivity to the explored dark matter models. We obtain constraints on the annihilation cross-section for different channels that are among the most robust and stringent achieved so far at the TeV mass scale from observations of dwarf satellite galaxies.

==> caption/CHANGELOG <==
caption package
===============

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added


bicaption package
=================

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added


ltcaption package
=================

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
==================

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption


newfloat package
================

v1.0 (2011/10/30)
- 1st published version

v1.1 (2013/04/27)
- New command \PrepareListOf


totalcount package
==================

v1.0 (2008/03/09)
- 1st published version



==> caption/README <==
==========================================================================

The `caption' package bundle
Release 2016-05-22
Copyright (C) 1994-2016 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  http://sourceforge.net/projects/latex-caption/

If you need help for installation please visit:
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=inst-miktex*
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=installthings
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=privinst

If you need help using these packages please visit:
  http://www.latex-community.org/
  http://tex.stackexchange.com/
  http://www.golatex.de/           (German)
  http://www.texwelt.de/           (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  http://sourceforge.net/p/latex-caption/tickets/
or send an e-mail to me
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.3 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption-eng.pdf (English)
             caption-rus.pdf (Russian, outdated)
             caption-deu.pdf (German)

--------------------------------------------------------------------------

The `bicaption' package v1.1 is a tiny package supporting the typesetting
of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.1 is a small package supporting typesetting
of sub-captions (by using the the sub-caption feature of the `caption'
package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

The `newfloat' package v1.1 offers the command \DeclareFloatingEnvironment
for defining new floating environments which behave like the existing
floating environments "figure" and "table".

User Manual: newfloat.pdf (English)

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)


==> liesmich <==
=> see  "readme"  for an  english  version of  this file <=

************************************************************
*                                                          *
*                     yfonts.sty v1.3                      *
*                                                          *
*     Ein Makropaket fuer den Fraktursatz mit LaTeX2e      *
*                                                          *
************************************************************
                                              Walter Schmidt
                                      <w-a-schmidt@arcor.de>
                                                  2003-01-08

Das Makropaket yfonts.sty ermoeglicht die Benutzung der von
Yannis Haralambous entworfenen altdeutschen Schriften
Gotisch, Schwabacher, Fraktur und der barocken Initialen mit
LaTeX2e.

Das Paket kann zusammen mit german.sty benutzt werden und
integriert die o.g.  Fonts trotz ihres unkonventionellen
Zeichenvorrats in LaTeX und das NFSS.  Ein Makro ermoeglicht
es, einen Absatz mit einer eingezogenen Initiale zu
beginnen.


LaTeX-Dateien
-------------
yfonts.dtx      LaTeX-Quelle
yfonts.ins      Installations-Skript
frktest.tex     kurzes Beispiel


Unterstuetzte Schriften
-----------------------
Das Paket yfonts.sty unterstuetzt folgende Fonts:

ygoth    Gotisch            aus  <ctan>/fonts/gothic/ygoth
yswab    Schwabacher             <ctan>/fonts/gothic/yswab
yfrak    Fraktur                 <ctan>/fonts/gothic/yfrak
ysmfrak  Fraktur (Variante)      <ctan>/fonts/gothic/yfrak
yinitas  Initialen               <ctan>/fonts/gothic/yinit

Wie obige Fonts installiert werden mussen, haengt vom
benutzten TeX-System ab und wird hier NICHT beschrieben,

*** WARNUNG *** WARNUNG *** WARNUNG *** WARNUNG *** WARNUNG

Bei der METAFONT-Bearbeitung der gotischen Schrift kann es
zu Fehlern kommen.  In wenigen Faellen wurden Probleme auch
mit den anderen Schriften beobachtet, offenbar abhaengig vom
"mode" und der Vergroesserung.  Das ist kein Problem des
Pakets yfonts.sty, sondern es wird durch fehlerhaften
Metafont-Code der Schriften verursacht.  

Bitte, senden Sie Fragen oder Fehlermeldungen zu diesem
Problem an Yannis Haralambous <yannis@fluxus-virus.com>, der
diese Schriften entworfen hat.


Installation des LaTeX-Pakets
-----------------------------
Legen Sie die Dateien yfonts.dtx und yfonts.ins in ein
gemeinsames Verzeichnis.  In einem TDS-kompatiblen
TeX-System sollte es das Verzeichnis

  texmf/source/latex/yfonts

sein.  Bearbeiten Sie das Installations-Skript yfonts.ins
mit LaTeX, um das Makropaket zu entpacken.  Falls das
Verzeichnis

  texmf/tex/latex/yfonts
             
existiert, und wenn docstrip richtig konfiguriert ist, wird 
das Paket automagisch in diesem Verzeichnis erzeugt.
Ansonsten versetzen Sie es manuell dorthin -- oder in ein
anderes Verzeichnis, wo LaTeX es findet.

Bearbeiten Sie yfonts.dtx mit LaTeX, um die Beschreibung des
Pakets zu erzeugen.

Bearbeiten Sie das File frktest.tex mit LaTeX, um ein 
Beispiel zu sehen.


Geschichte
----------
v1.3 <2бб3-01-08>  Makros \AA und \aa funktionieren wieder.

v1.2 <1999-05-12>  Geaenderte Lizenzbedingung: LPPL

v1.2 <1998-10-03>  Neu: \yinipar (Dank an Bernd Raichle fuer
                   seinen Verbesserungsvorschlag!)
                   
v1.1 <1997-09-11>


% finis



==> readme <==
=> dieser Text in deutscher Sprache:    Datei "liesmich" <=

************************************************************
*                                                          *
*                     yfonts.sty v1.3                      *
*                                                          *
*    A package for using old german fonts with LaTeX2e     *
*                                                          *
************************************************************
                                              Walter Schmidt
                                      <w-a-schmidt@arcor.de>
                                                  2003-01-08

The macro package "yfonts" provides a LaTeX interface to the
blackletter (old german) fonts designed by Yannis
Haralambous:  Gotisch, Schwabacher, Fraktur and the baroque
initials.

Despite their non-standard encoding, these fonts are fully
integrated into LaTeX's font management (NFSS), and the
package can be used together with german.sty.  A macro is
provided which starts a paragraph with an embedded initial.


LaTeX files
-----------
yfonts.dtx      LaTeX source
yfonts.ins      installation script
frktest.tex     short example


The fonts
---------
The package yfonts.sty supports the following fonts:

ygoth    Gotisch            from <ctan>/fonts/gothic/ygoth
yswab    Schwabacher             <ctan>/fonts/gothic/yswab
yfrak    Fraktur                 <ctan>/fonts/gothic/yfrak
ysmfrak  Fraktur (variant)       <ctan>/fonts/gothic/yfrak
yinitas  initials                <ctan>/fonts/gothic/yinit

It depends on your TeX system, how the above fonts are to be
installed.  This topic is NOT discussed here.

*** WARNING *** WARNING *** WARNING *** WARNING *** WARNING 

The font "ygoth" is known to produce Metafont errors.  In
rare cases such problems have been observed with the other
fonts, too.  This has nothing to do with the package
yfonts.sty, it is due to incorrect Metafont code of the
fonts.  

Questions and bug reports on this problem should be sent 
to Yannis Haralambous <yannis@fluxus-virus.com>, who has
designed the old german fonts.


Installing the LaTeX package
----------------------------
Put the files yfonts.dtx and yfonts.ins into a common
directory.  On a TDS-compliant TeX system, use:

  texmf/source/latex/yfonts

Run LaTeX on yfonts.ins to generate the macro package file
yfonts.sty.  Move it to a directory where TeX searches for
input files; in a TDS compliant system this should be:

  texmf/tex/latex/yfonts

If you have properly set up your docstrip program and the
above directory exists already, this is done automagically!

Run LaTeX on yfonts.dtx to typeset the documentation of the
LaTeX package.  The documentation is written in german, so
you will need german.sty and the german hyphenation
patterns.

Run LaTeX on the example frktest.tex to see an example using
the blackletter fonts; again, german.sty is required.


A short (and incomplete) english guide to yfonts.sty
----------------------------------------------------
The commands \gothfamily, \swabfamily, \frakfamily and
\initfamily switch to Gotisch, Schwabacher, Fraktur or
initials within the current group.

\textgoth{...}, \textswab{...},  \textfrak{...} and 
\textinit{...} typeset their argument using old german 
fonts.

Size changing command are honored; available sizes are 10pt, 
10.95pt, 12pt ... 24.88pt.

There are no further font series or shapes.  You may however
use Schwabacher for emphasizing within a Fraktur
environment, thus following historical practice.

The regular \baselineskip is too large for the old german
fonts; the command \fraklines selects a suitable
\baselineskip for Fraktur or Schwabacher within the current
group; you must repeat it after any size changing command.

Some ASCII symbols are missing (there is e.g. no ";" in the 
Schwabacher font, and none of the fonts has a "@")

A paragraph in Fraktur which starts with an embedded
initial:
 
  {\frakfamily\fraklines
   \yinipar{E}in Absatz ...
   
   \par
  }

\yinipar begins a new paragraph (like \par) and suppresses
indentation (like \noindent).  The end of the paragraph
(blank line or \par) must be within in the same group as the
command \fraklines.

Use the regular LaTeX commands for umlauts, accents and
special symbols.  You may additionally load german.sty.

Important ligatures:

  *a *e *o *u produce a special version of the umlauts with 
  a small e instead of the dots. Load the package with the
  option [varumlaut] to get them with the regular commands,
  like \"a or "a, too.

  s: is the so-called final s

  the sharp s may be produced by \ss, "s or the ligature sz

The command \etc produces a once popular symbol for "etc.";
it is available in the Fraktur font only.


History
-------
v1.3 <2003-01-08> \AA and \aa fixed.

v1.2 <1999-05-12> License agreement changed to LPPL.

v1.2 <1998-09-10> New: \yinipar

v1.1 <1997-09-11>


% finis



==> yfonts/liesmich <==
=> see  "readme"  for an  english  version of  this file <=

************************************************************
*                                                          *
*                     yfonts.sty v1.3                      *
*                                                          *
*     Ein Makropaket fuer den Fraktursatz mit LaTeX2e      *
*                                                          *
************************************************************
                                              Walter Schmidt
                                      <w-a-schmidt@arcor.de>
                                                  2003-01-08

Das Makropaket yfonts.sty ermoeglicht die Benutzung der von
Yannis Haralambous entworfenen altdeutschen Schriften
Gotisch, Schwabacher, Fraktur und der barocken Initialen mit
LaTeX2e.

Das Paket kann zusammen mit german.sty benutzt werden und
integriert die o.g.  Fonts trotz ihres unkonventionellen
Zeichenvorrats in LaTeX und das NFSS.  Ein Makro ermoeglicht
es, einen Absatz mit einer eingezogenen Initiale zu
beginnen.


LaTeX-Dateien
-------------
yfonts.dtx      LaTeX-Quelle
yfonts.ins      Installations-Skript
frktest.tex     kurzes Beispiel


Unterstuetzte Schriften
-----------------------
Das Paket yfonts.sty unterstuetzt folgende Fonts:

ygoth    Gotisch            aus  <ctan>/fonts/gothic/ygoth
yswab    Schwabacher             <ctan>/fonts/gothic/yswab
yfrak    Fraktur                 <ctan>/fonts/gothic/yfrak
ysmfrak  Fraktur (Variante)      <ctan>/fonts/gothic/yfrak
yinitas  Initialen               <ctan>/fonts/gothic/yinit

Wie obige Fonts installiert werden mussen, haengt vom
benutzten TeX-System ab und wird hier NICHT beschrieben,

*** WARNUNG *** WARNUNG *** WARNUNG *** WARNUNG *** WARNUNG

Bei der METAFONT-Bearbeitung der gotischen Schrift kann es
zu Fehlern kommen.  In wenigen Faellen wurden Probleme auch
mit den anderen Schriften beobachtet, offenbar abhaengig vom
"mode" und der Vergroesserung.  Das ist kein Problem des
Pakets yfonts.sty, sondern es wird durch fehlerhaften
Metafont-Code der Schriften verursacht.  

Bitte, senden Sie Fragen oder Fehlermeldungen zu diesem
Problem an Yannis Haralambous <yannis@fluxus-virus.com>, der
diese Schriften entworfen hat.


Installation des LaTeX-Pakets
-----------------------------
Legen Sie die Dateien yfonts.dtx und yfonts.ins in ein
gemeinsames Verzeichnis.  In einem TDS-kompatiblen
TeX-System sollte es das Verzeichnis

  texmf/source/latex/yfonts

sein.  Bearbeiten Sie das Installations-Skript yfonts.ins
mit LaTeX, um das Makropaket zu entpacken.  Falls das
Verzeichnis

  texmf/tex/latex/yfonts
             
existiert, und wenn docstrip richtig konfiguriert ist, wird 
das Paket automagisch in diesem Verzeichnis erzeugt.
Ansonsten versetzen Sie es manuell dorthin -- oder in ein
anderes Verzeichnis, wo LaTeX es findet.

Bearbeiten Sie yfonts.dtx mit LaTeX, um die Beschreibung des
Pakets zu erzeugen.

Bearbeiten Sie das File frktest.tex mit LaTeX, um ein 
Beispiel zu sehen.


Geschichte
----------
v1.3 <2бб3-01-08>  Makros \AA und \aa funktionieren wieder.

v1.2 <1999-05-12>  Geaenderte Lizenzbedingung: LPPL

v1.2 <1998-10-03>  Neu: \yinipar (Dank an Bernd Raichle fuer
                   seinen Verbesserungsvorschlag!)
                   
v1.1 <1997-09-11>


% finis



==> yfonts/readme <==
=> dieser Text in deutscher Sprache:    Datei "liesmich" <=

************************************************************
*                                                          *
*                     yfonts.sty v1.3                      *
*                                                          *
*    A package for using old german fonts with LaTeX2e     *
*                                                          *
************************************************************
                                              Walter Schmidt
                                      <w-a-schmidt@arcor.de>
                                                  2003-01-08

The macro package "yfonts" provides a LaTeX interface to the
blackletter (old german) fonts designed by Yannis
Haralambous:  Gotisch, Schwabacher, Fraktur and the baroque
initials.

Despite their non-standard encoding, these fonts are fully
integrated into LaTeX's font management (NFSS), and the
package can be used together with german.sty.  A macro is
provided which starts a paragraph with an embedded initial.


LaTeX files
-----------
yfonts.dtx      LaTeX source
yfonts.ins      installation script
frktest.tex     short example


The fonts
---------
The package yfonts.sty supports the following fonts:

ygoth    Gotisch            from <ctan>/fonts/gothic/ygoth
yswab    Schwabacher             <ctan>/fonts/gothic/yswab
yfrak    Fraktur                 <ctan>/fonts/gothic/yfrak
ysmfrak  Fraktur (variant)       <ctan>/fonts/gothic/yfrak
yinitas  initials                <ctan>/fonts/gothic/yinit

It depends on your TeX system, how the above fonts are to be
installed.  This topic is NOT discussed here.

*** WARNING *** WARNING *** WARNING *** WARNING *** WARNING 

The font "ygoth" is known to produce Metafont errors.  In
rare cases such problems have been observed with the other
fonts, too.  This has nothing to do with the package
yfonts.sty, it is due to incorrect Metafont code of the
fonts.  

Questions and bug reports on this problem should be sent 
to Yannis Haralambous <yannis@fluxus-virus.com>, who has
designed the old german fonts.


Installing the LaTeX package
----------------------------
Put the files yfonts.dtx and yfonts.ins into a common
directory.  On a TDS-compliant TeX system, use:

  texmf/source/latex/yfonts

Run LaTeX on yfonts.ins to generate the macro package file
yfonts.sty.  Move it to a directory where TeX searches for
input files; in a TDS compliant system this should be:

  texmf/tex/latex/yfonts

If you have properly set up your docstrip program and the
above directory exists already, this is done automagically!

Run LaTeX on yfonts.dtx to typeset the documentation of the
LaTeX package.  The documentation is written in german, so
you will need german.sty and the german hyphenation
patterns.

Run LaTeX on the example frktest.tex to see an example using
the blackletter fonts; again, german.sty is required.


A short (and incomplete) english guide to yfonts.sty
----------------------------------------------------
The commands \gothfamily, \swabfamily, \frakfamily and
\initfamily switch to Gotisch, Schwabacher, Fraktur or
initials within the current group.

\textgoth{...}, \textswab{...},  \textfrak{...} and 
\textinit{...} typeset their argument using old german 
fonts.

Size changing command are honored; available sizes are 10pt, 
10.95pt, 12pt ... 24.88pt.

There are no further font series or shapes.  You may however
use Schwabacher for emphasizing within a Fraktur
environment, thus following historical practice.

The regular \baselineskip is too large for the old german
fonts; the command \fraklines selects a suitable
\baselineskip for Fraktur or Schwabacher within the current
group; you must repeat it after any size changing command.

Some ASCII symbols are missing (there is e.g. no ";" in the 
Schwabacher font, and none of the fonts has a "@")

A paragraph in Fraktur which starts with an embedded
initial:
 
  {\frakfamily\fraklines
   \yinipar{E}in Absatz ...
   
   \par
  }

\yinipar begins a new paragraph (like \par) and suppresses
indentation (like \noindent).  The end of the paragraph
(blank line or \par) must be within in the same group as the
command \fraklines.

Use the regular LaTeX commands for umlauts, accents and
special symbols.  You may additionally load german.sty.

Important ligatures:

  *a *e *o *u produce a special version of the umlauts with 
  a small e instead of the dots. Load the package with the
  option [varumlaut] to get them with the regular commands,
  like \"a or "a, too.

  s: is the so-called final s

  the sharp s may be produced by \ss, "s or the ligature sz

The command \etc produces a once popular symbol for "etc.";
it is available in the Fraktur font only.


History
-------
v1.3 <2003-01-08> \AA and \aa fixed.

v1.2 <1999-05-12> License agreement changed to LPPL.

v1.2 <1998-09-10> New: \yinipar

v1.1 <1997-09-11>


% finis


